Dynamic-Net: Tuning the Objective Without Re-training for Synthesis Tasks

One of the key ingredients for successful optimization of modern CNNs is identifying a suitable objective. To date, the objective is fixed a-priori at training time, and any variation to it requires re-training a new network. In this paper we present a first attempt at alleviating the need for re-training. Rather than fixing the network at training time, we train a "Dynamic-Net" that can be modified at inference time. Our approach considers an "objective-space" as the space of all linear combinations of two objectives, and the Dynamic-Net is emulating the traversing of this objective-space at test-time, without any further training. We show that this upgrades pre-trained networks by providing an out-of-learning extension, while maintaining the performance quality. The solution we propose is fast and allows a user to interactively modify the network, in real-time, in order to obtain the result he/she desires. We show the benefits of such an approach via several different applications.

==> figures/fig_single_vs_multi_block.tex <==
\begin{figure}
\centering
%\includegraphics[width=0.7\linewidth]{style_transfer_images/brad_pitt_multi_vs_single_v2.PNG}
\includegraphics[width=0.85\linewidth]{style_transfer_images/brad_pitt_multi_vs_single_v7.PNG}
% \fboxsep=0mm%padding thickness
% \fboxrule=1pt%border thickness
% \definecolor{green_v1}{RGB}{84,130,53}
% \definecolor{purple_v1}{RGB}{112,48,160}
% \setlength{\tabcolsep}{0pt}
% \begin{tabular}{c c c c}
%      \fcolorbox{green_v1}{green_v1}{\includegraphics[width=0.2\linewidth]{style_transfer_images/multi_vs_single/multi_000.jpg}} &
%      \fcolorbox{green_v1}{green_v1}{\includegraphics[width=0.2\linewidth]{style_transfer_images/multi_vs_single/multi_025.jpg}} &
%      \fcolorbox{green_v1}{green_v1}{\includegraphics[width=0.2\linewidth]{style_transfer_images/multi_vs_single/multi_050.jpg}} &
%      \fcolorbox{green_v1}{green_v1}{\includegraphics[width=0.2\linewidth]{style_transfer_images/multi_vs_single/multi_100.jpg}} 
%      \\
%      \fcolorbox{purple_v1}{purple_v1}{\includegraphics[width=0.2\linewidth]{style_transfer_images/multi_vs_single/single_000.jpg}} &
%      \fcolorbox{purple_v1}{purple_v1}{\includegraphics[width=0.2\linewidth]{style_transfer_images/multi_vs_single/single_030.jpg}} &
%      \fcolorbox{purple_v1}{purple_v1}{\includegraphics[width=0.2\linewidth]{style_transfer_images/multi_vs_single/single_060.jpg}} &
%      \fcolorbox{purple_v1}{purple_v1}{\includegraphics[width=0.2\linewidth]{style_transfer_images/multi_vs_single/single_100.jpg}}
% \end{tabular}
\vspace{-0.3cm}
\caption{\textbf{Single- vs. multi- block framework:}
The multi-block framework allow us to use the set $\alpha^l$ for tuning -- a scan over $21^3$ values of $\alpha^l$ is shown by the green plain. In contrast, training a single-block produce only a single curve (blue and purple) in the objective space. In many cases, both frameworks, purple curve and the lower bound of the green plain, achieve similar approximation of the fixed nets, marked by $\times$. We also show robustness to the location of the tuning-block, the blue curve and purple curve correspond to different locations of the tuning-block in the network.
% \textbf{Bottom:} example images of the
% We show also the curve we get when $\alpha^0\!=\!\alpha^1\!=\!\alpha^2$ (green). The images show two versions of the single-block framework, where we trained only the 1st/2nd tuning-block of the multi-block framework. 
% All setting of our method were trained with the same objective
% ($ \lambda_0\!=\!2\cdot10^4 $, $ \lambda_1\!=\!10^7 $).
}
\label{fig:single_vs_multi_block}
\end{figure}


==> figures/fig_style_transfer_feathers_van.tex <==
\begin{figure*}
\centering
\begin{tabular}{c c}
\includegraphics[width=0.7\linewidth]{style_transfer_images/ours_vs_blending_van_1e5_1e7.jpg}
\includegraphics[width=0.3\linewidth]{style_transfer_images/feathers_van_1e5_1e7.png}\\
\includegraphics[width=0.7\linewidth]{style_transfer_images/ours_vs_blending_van_1e5_2e4.jpg}
\includegraphics[width=0.3\linewidth]{style_transfer_images/feathers_van_1e5_2e4.png}
\end{tabular}
\caption{\textbf{First row:} Our solution results (red line in graph, increasing $ \alpha=\beta=\gamma $). \textbf{second row:} Base line result, blending of two networks (first: $ \lambda = 10^5 $, second: $ \lambda = 10^6 $, second blue line in graph). \textbf{Third row:} Our solution results (red line in graph, increasing $ \alpha=\beta=\gamma $). \textbf{forth row:} Base line result, blending of two networks (first: $ \lambda = 2*10^4 $, second: $ \lambda = 10^5 $, orange line in graph). Red lines in graphs correspond to our solution while $ \alpha = \beta = \gamma $, strong blue line correspond to blending network output of $ \alpha = 0 $ and $ alpha = 1 $.}
\label{fig:feathers_van}
\end{figure*}
